Improving Phase Change Memory Performance with Data Content Aware Access

A prominent characteristic of write operation in Phase-Change Memory (PCM) is that its latency and energy are sensitive to the data to be written as well as the content that is overwritten. We observe that overwriting unknown memory content can incur significantly higher latency and energy compared to overwriting known all-zeros or all-ones content. This is because all-zeros or all-ones content is overwritten by programming the PCM cells only in one direction, i.e., using either SET or RESET operations, not both. In this paper, we propose data content aware PCM writes (DATACON), a new mechanism that reduces the latency and energy of PCM writes by redirecting these requests to overwrite memory locations containing all-zeros or all-ones. DATACON operates in three steps. First, it estimates how much a PCM write access would benefit from overwriting known content (e.g., all-zeros, or all-ones) by comprehensively considering the number of set bits in the data to be written, and the energy-latency trade-offs for SET and RESET operations in PCM. Second, it translates the write address to a physical address within memory that contains the best type of content to overwrite, and records this translation in a table for future accesses. We exploit data access locality in workloads to minimize the address translation overhead. Third, it re-initializes unused memory locations with known all-zeros or all-ones content in a manner that does not interfere with regular read and write accesses. DATACON overwrites unknown content only when it is absolutely necessary to do so. We evaluate DATACON with workloads from state-of-the-art machine learning applications, SPEC CPU2017, and NAS Parallel Benchmarks. Results demonstrate that DATACON significantly improves system performance and memory system energy consumption compared to the best of performance-oriented state-of-the-art techniques.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> sections/junk.tex <==
For easy access, 

so that they can be used to service write requests.

The first component is a \emph{status table} (ST), which stores the status of the physical locations in PCM. 
%We organize ST as a fully associative structure. 
A physical memory location can be in one of the four states: (1) \emph{unused}, (2) {used in some address translation}, (3) \emph{initialized} to all-zeros, and (4) \emph{initialized} to all-ones.
\mcfive{
The second component is a fully-associative
\emph{address translation table} (AT). 
Each entry in this table stores the physical memory address for the corresponding write address generated from the eDRAM cache.
%holds the translated address of the address pointed by the index to this table.
%We organize AT as a fully associative structure to facilitate indirection-based address translation. To reduce the area overhead of AT, we also propose an alternative scheme to organize AT for content-based address translation. 
The third component is an \emph{initialization queue} (InitQ), which is used to schedule the all-0s or all-1s re-initialization of unused memory locations so that future PCM writes can be serviced utilizing them.
}

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.99\columnwidth]{images/address_translation_overview_diagram.pdf}}
	\caption{\mcfive{\tech{}'s address translation mechanism.}}
	\label{fig:att}
\end{figure}

\mcfive{
Figure~\ref{fig:at_st} illustrates the operation of \tech{} while servicing PCM reads and writes. To service a read request, \tech{} translates the read address to a physical address in PCM using the AT. In this example, the address {0x30a} for the read request coming from the request queue is translated to the physical address {0x11fe} and directed to PCM. The ST entry of 0x11fe is 1 indicating that the address is used in some translation (to translate 0x30a in this example), which is recorded in AT. The original read address (0x30a) is re-initialized to all-1s and is indicated by the ST entry of 3.
}

\mcfive{
To service a write request, \tech{} first searches the ST for an all-0s initialized PCM location based on the write data. In Section \ref{sec:prioritization} we illustrate how to choose between all-0s and all-1s content based on the write data. Looking at the ST we see that location 0x91004b is initialized to all-0s. Therefore, the write address 0x1078 is translated to the physical address 0x91004b and the write request is directed to PCM. The address translation of write address 0x1078 to physical address 0x91004b is recorded in AT. In this way, any future read requests to 0x1078 are redirected to the new physical address 0x91004b in PCM.
To use the original write address 0x1078 in servicing some future write request, we invalidate this address in ST by setting the corresponding entry to 0 as illustrated in this example. In Section \ref{sec:scheduling} we describe how we re-initialize unused PCM locations.
%to service future read requests to this write address. Since the write address is no longer 
}

\mcfive{
Finally, fully-associative address translation table leads to high area overhead in storing the ST and AT inside the memory controller. In Section \ref{sec:translation} we describe a caching policy, which reduces this overhead.
}

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=0.99\columnwidth]{images/AT_ST.pdf}}
	\caption{\mcfive{Illustration of \tech{}'s address translation mechanism for servicing PCM reads and writes.}}
	\label{fig:at_st}
\end{figure}

We now describe the three operations of \tech.%~in more detail.

%Our architectural technique, \tech, reduces the energy and latency of PCM writes.
%% by overwriting, whenever possible, memory locations containing all zeros and all ones.
%This is achieved by dynamically redirecting write requests to memory locations containing known data pattern e.g., all zeros, or all ones as much as possible.
%Only when no such locations can be found in PCM, is an unknown content overwritten. 
%Our architectural technique has three key components -- \textbf{\emph{content selection}} (selecting between overwriting all zeros, all ones, and unknown content), \textbf{\emph{address translation}} (redirecting a write request to the memory location containing the selected content), and \textbf{\emph{request scheduling}} (periodically reinitializing unused memory locations with all zeros or all ones data pattern such that these can be used to service PCM writes as much as possible).
%
%
%To this end, a table is used to store the status of the physical locations in PCM.
%Each entry of this table is a 2-bit register encoding the status as follows.
%\begin{itemize}
%	\item {00:} the content is unused,
%	\item {01:} the content is uninitialized and valid,
%	\item {10:} the content is initialized to all zeros, and
%	\item {11:} the content is initialized to all ones.
%\end{itemize} 
%The status table is updated during a write request and also when a memory location is initialized.
%
%%, indicating whether theirs contents are all zeros or all ones.
%%On eviction from the cache using writeback or writethrough policy, a dirty cache line is written back to the PCM.
%%The write data is first analyzed to select between overwriting all zeros and all ones.
%%is to be written back to the PCM on eviction from the cache (writeback or writethrough),
%When a dirty cache line is evicted from the cache, the write data is first analyzed to select between overwriting all zeros and all ones data pattern.
%Based on this selection and the content of the status table, a memory location is identified to service the write. 
%%
%%selected such that the write request can now be serviced with low energy and latency by programming in one direction only i.e., either SET or RESET of the memory cells, rather than both.
%%identified for servicing the write.
%The write request is redirected to this location by translating its write address to the physical address. %of the selected memory location. % and will be serviced with low energy and latency due to programming in one direction only i.e., either SET or RESET of the memory cells, rather than both.
%%The write request will now be serviced with low energy and latency due to programming in one direction only i.e., either SET or RESET of the memory cells, rather than both.
%A lookup table is used to track the dynamic address translations.
%%While servicing a read request, the read address is translated to the correct physical address using the lookup table.
%We propose a new scheduling policy that reclaims i.e., reinitializes unused memory locations with all zeros or all ones data pattern whenever possible, such that these locations can be used to service future write requests.
%
%The remainder of this section is organized as follows.
%We describe our prioritization policy for selecting between all zeros and all ones memory location in Section \ref{sec:prioritization}.
%We proposed different address translation strategies in Section \ref{sec:translation}.
%We describe our scheduling policy for initializing unused memory locations in Section \ref{sec:scheduling}.
%%Finally, we describe how \tech~improves system performance by allowing to read and write from the same memory partition in Section \ref{sec:read_while_write}.

%\subsection{Selecting Between Overwriting All Zeros and All Ones Memory Content}
\subsubsection{Selecting the Overwritten Content}
\label{sec:prioritization}
\mcfive{
Figure \ref{fig:flowchart} illustrates \tech{}'s policy to select the overwritten content for every PCM write request. 
If the number of SET bits in the write data is more than 60\%, \tech{} checks the status table to see if there is all-0s or all-1s locations available in PCM.
%are memory locations in PCM that are initialized to all-0s or all-1s. 
If an all-1s location is available, \tech{} selects it as the overwritten content. This is because overwriting all-1s using RESET operations is both more energy efficient and higher performance than overwriting any other content when the fraction of SET bits in the write data is more than 60\%. In this way, \tech{} optimizes both \emph{performance and energy}.
Otherwise, if an all-0s location is available, \tech{} selects it as the overwritten content. This is because overwriting all-0s using SET programming has lower latency than overwriting unknown content. In this way, \tech{} optimizes \emph{performance}.  %However, if there is no all-0s or all-1s location available, \tech{} does not translate write address, thereby overwriting unknown content.
}

\mcfive{
Conversely, if the number of SET bits in the write data is less than 60\% and there is an all-0s location available, \tech{} selects it as the overwritten content. This is because overwriting all-0s using SET programming is more energy efficient than overwriting any other content when the fraction of SET bits in the write data is less than 60\%. In this way,  \tech{} optimizes \emph{energy}. Otherwise, if an all-1s location is available, \tech{} selects it as the overwritten content. This is because overwriting all-1s using RESET programming has lower latency than overwriting unknown content. 
 In this way, \tech{} optimizes \emph{performance}. 
%If there is no all-0s or all-1s location available, \tech{} does not translate write address, thereby overwriting unknown content.
}

\tech{} overwrites the existing content, which is unknown at the time of a PCM write only if there are no all-0s or all-1s locations available in PCM to service the write request. %Otherwise, \tech{} improves performance and energy consumption by overwriting all-0s or all-1s based on the write data.


% When a PCM write request is generated, DATACON calculates three priorities: (1) the priority to overwrite all-zeros, (2) the priority to overwrite all-ones, and (3) the priority to overwrite the existing memory content, which is unknown at the time of servicing the write request.
% %the current content, which is unknown at the time of write.
% %The priority is computed based on the energy and that status of the initialized contents in the PCM. 
% We estimate these priorities as follows.

\begin{figure}[h!]
 	\centering
    %\vspace{-10pt}
 	\centerline{\includegraphics[width=0.99\columnwidth]{images/flowchart.pdf}}
 	\vspace{-10pt}
 	\caption{\mcfive{Flowchart for selecting the overwritten data.}}
    %\vspace{-10pt}
 	\label{fig:flowchart}
\end{figure}

% We consider a $N\times W$ PCM bank with $N$ rows, each with $W$ PCM cells. 
% %Let each memory location in PCM consists of $W$ PCM cells. 
% %We denote the write data by $D$.
% % be the write data to be written to a memory location consisting of $W$ PCM cells. 
% The energy consumed to overwrite all-ones using the write data $D$ is
% \begin{equation}
% \label{eq:siw_energy}
% \scriptsize E_{\text{1}} = W*E_{\text{SET}} + \left[W-\texttt{popcount(D)}\right]*E_{\text{RESET}}
% \end{equation}
% %\begin{equation}
% %\label{eq:siw_latency}
% %\scriptsize L_{\text{SIW}} = L_{\text{XOR}} + L_{\text{RESET}}
% %\end{equation}
% where $E_{\text{SET}}$ and $E_{\text{RESET}}$ are the energy consumed for the SET and RESET operations of a PCM cell, respectively, and $\texttt{popcount(D)}$ computes the number of set bits in $D$. 
% In the above expression, the term $W*E_{\text{SET}}$ is the preparation energy required to initialize a row with all-ones. The energy consumed to overwrite all-zeros using the same write data is 
% \begin{equation}
% \label{eq:riw_energy}
% \scriptsize E_{\text{0}} = W*E_{\text{RESET}} + \texttt{popcount(D)}*E_{\text{SET}}
% \end{equation}

% %Let $N_0$ and $N_1$ be the number of all zeros and all ones locations in the PCM, respectively. 
% We express the  three dynamic priorities as follows.
% \begin{equation}
% \label{eq:priority_0}
% \scriptsize P_\text{all\_zeros} = \frac{E_\text{1}}{E_\text{0}}\times \widehat{N_0}~~~~\text{//to overwrite all zeros}
% \end{equation}
% \begin{equation}
% \label{eq:priority_1}
% \scriptsize P_\text{all\_ones} = \frac{E_\text{0}}{E_\text{1}}\times \widehat{N_1}~~~~\text{//to overwrite all ones}
% \end{equation}
% \begin{equation}
% \label{eq:priority_unknown}
% \scriptsize P_\text{unknown} = (1-\widehat{N_0})\times(1-\widehat{N_1})~~~~\text{//to overwrite unknown content}
% \end{equation}
% where $\widehat{N_0}$ and $\widehat{N_1}$ are the binary variables that indicate the presence of all-zeros and all-ones rows in PCM, respectively. %These binary indicators are computed as follows.
% %\begin{equation}
% %\label{eq:n0_n1}
% %\scriptsize \widehat{N_0} = \begin{cases}
% %1, & \text{for } N_0 \geq 1 \\
% %0, & \text{otherwise }
% %\end{cases} \text{ and } \widehat{N_1} = \begin{cases}
% %1, & \text{for } N_1 \geq 1 \\
% %0, & \text{otherwise }
% %\end{cases}
% %\end{equation}
% We now describe the selection of the \emph{best} overwritten content based on these priorities. 

% In Table \ref{tab:priority}, we summarize DATACON's content selection criteria.
% We make four key observations from this table.
% %write requests are redirected appropriately as summarized in Table \ref{tab:priority}.

% \begin{table}[h!]
% 	\centering
% 	{\fontsize{6}{10}\selectfont
% 		\begin{tabular}{|c||c|c|c||c|c|}
% 			\hline
% 			\multirow{2}{*}{\textbf{Criterion}} & \multirow{2}{*}{\textbf{Energy}} & \multirow{2}{*}{$\mathbf{\widehat{N_0}}$} & \multirow{2}{*}{$\mathbf{\widehat{N_1}}$} & \textbf{Overwritten} &	\multirow{2}{*}{\textbf{Priority}}\\
% 			&&&&\textbf{content} &\\
% 			\hline
% 			\hline
% 			1 & \multirow{2}{*}{$E_{\text{0}} < E_{\text{1}}$} & $1$ & $\geq0$ & all-zeros & Energy\\
% 			2 & & $0$ & $\geq1$ & all-ones & Latency\\
% 			\hline
% 			3 & \multirow{2}{*}{$E_{\text{1}} < E_{\text{0}}$} & $\geq 0$ & $1$ & all-ones & Energy\\
% 			4 & & $\geq 1$ & $0$ & all-zeros & Latency\\
% 			\hline
% 			\multirow{2}{*}{5} & $E_{\text{0}} < E_{\text{1}}$ or & \multirow{2}{*}{0} & \multirow{2}{*}{0} & \multirow{2}{*}{existing (unknown)} & \multirow{2}{*}{--}\\
% 			& $E_{\text{1}} < E_{\text{0}}$  & & & &\\
% 			\hline
% 	\end{tabular}}
% 	\caption{Overwritten content selection.}
% 	\label{tab:priority}
% \end{table}
% %, which shows that \tech the existing content, which is \emph{unknown} at the time of the write request is selected as the overwritten content.

% \changed{First, when there are available rows with all-zeros and all-ones content, \tech~reduces the latency and energy of PCM writes by selecting one of these contents (criteria 1-4 in the table). Between all-zeros and all-ones content, one is prioritized over the other based on (1) the total energy, which incorporates the number of set bits in the write data, and the energy of SET and RESET operations in PCM (see Equations \ref{eq:siw_energy} \& \ref{eq:riw_energy}), and (2) SET and RESET latency required to overwrite all-zeros and all-ones content, respectively.}

% \changed{Second, if there are available rows with all-zeros content and the energy overhead of overwriting all-zeros is lower than overwriting all-ones, then \tech~selects all-zeros as the overwritten content (criterion 1). Conversely, \tech~selects all-ones as the overwritten content when there are rows with all-ones content available in PCM, and overwriting all-ones is more energy efficient than overwriting all-zeros (criterion 3).}
% \changed{Third, if overwriting all-zeros is more energy efficient than overwriting all-ones, but only all-ones rows are available, DATACON selects all-ones as the overwritten content, rather than the existing content (criterion 2). This is because overwriting all-ones with only RESET operations incurs significantly lower latency than overwriting unknown contents, which requires both SET and RESET operations. Conversely, \tech~selects all-zeros content as the overwritten content, if these are only all-zeros rows available in the PCM (criterion 4).}

% \changed{Finally, \tech~overwrites the existing content, wh\-ich is unknown at the time of the write request, \emph{only when} there are \emph{no} row with all-zeros or all-ones content available in PCM (criterion 5).}

% For all other conditions, \tech~selects 
%From Equations \ref{eq:priority_0}-\ref{eq:priority_unknown}, we see that an unknown content is overwritten only when $\widehat{N_0}$ and $\widehat{N_1}$ are both zero, i.e., when there are no all zeros and all ones content in the memory. 
%This is captured in the final row in Table \ref{tab:priority}. 
%Otherwise, \tech~reduces write latency and energy by assigning \emph{non-zero} priorities to overwrite all-zeros and all-ones content, and a \emph{zero} priority to overwrite the existing (i.e., unknown) content. 
%Between overwriting all-zeros and all-ones, one is assigned a higher priority than the other based on the energy ratio, which is estimated from Equations \ref{eq:siw_energy} \& \ref{eq:riw_energy}. %the number of set bits in the write data.%, the presence of all zeros and all ones locations in PCM.
%
%Second, we observe from row 4 that although overwriting all-zeros is energy efficient than overwriting all-ones, there are no all-zeros memory location available in PCM ($\widehat{N_0} = 0$).
%% for the third condition in Table \ref{tab:priority}, there are no all zero locations available in the PCM ($N_0 = 0$).
%In this case, DATACON prioritizes overwriting all-ones over overwriting an unknown content, to \emph{reduce} the {write latency}.
%%there are two choices -- one to overwrite all ones and another to overwrite an unknown content.
%%We prioritize overwriting all ones to reduce the write latency. 
%%By doing so, DATACON incorporates write latency, in addition to write energy, when selecting the best overwritten content for a write request.

\subsubsection{Translating the Address of a Write Request}
\label{sec:translation}
Once the best overwritten content is decided, the next task is to select the physical address in PCM that contains this overwritten content. This is described next.

\tech~first searches the status table to find a list of rows, which contain the best overwritten content for the write data. 
An important question to this end is \emph{which} row from this list to assign to the write request.
While deciding this, \tech~checks the read queue.
If the read queue is empty, \tech~randomly selects a row from the list.
Otherwise, \tech~ensures that the chosen row belongs to 
a partition that is not serving any read requests. In this way, \tech{} can schedule the write request in parallel with an ongoing read request, exploiting the parallelism in PCM banks \cite{lung2016double,villa2018pcm}. Once the physical address is identified, the memory controller updates the AT to record this new address translation.

\mcfive{
As write requests are continuously remapped to different physical locations in PCM, the size of AT can be extremely large. To limit the area overhead of \tech{}, we propose 
to cache a part of the AT containing the address translation of recently accessed PCM partitions as a lookup table (LUT) inside the memory controller, while maintaining the entire AT inside PCM.
Figure~\ref{fig:att} illustrates this caching mechanism. 
%For each request in the read and write queue, the memory controller first checks to see if the translation for the memory address exists in the LUT. If it exists, the memory address of the request is translated to a physical address and scheduled to PCM. Otherwise, a PCM request is generated to first read the translation for the accessed partition into the LUT before translating the memory address and servicing the request.
}



\mcfive{
We implement the LUT to store address translations for \ineq{N} most recently used PCM partitions. We evaluate the performance impact of \ineq{N} in Section \ref{sec:caching}. 
% Under this new caching mechanism, the memory
% controller categorizes each PCM request into one of two cases: 1) \emph{LUT hit:}, i.e., the translation of the request's memory address is in the LUT, and ii) \emph{LUT miss:}, i.e., the translation of the request's memory address is not in LUT.
% In the first case, the memory address is translated using the translation from the LUT and the request is scheduled to PCM.
% In the second case, the memory controller issues a PCM request to read the address translation inside the LUT. To make space, the translations for the least recently used (LRU) PCM partition is evicted from the LUT. If the evicted content is dirty, i.e., updated, a PCM request is generated to write the updated content into PCM.
}

{
In our mechanism, we store the full AT in a separate PCM partition. In this way, any request to access AT following a LUT miss can be serviced in parallel to PCM reads and writes exploiting a PCM bank's partition-level parallelism~\cite{song2019enabling}. We illustrate this in Figure~\ref{fig:att}.
}
%an \emph{idle} partition in the PCM bank, one that is \emph{not} being utilized to service any current or pending read requests. By doing so, \tech~allows the read requests to be scheduled \emph{concurrently} with the write request by controlling the directions of the transmission gates in the \emph{decoupled read and verify} sense amplifiers in the peripheral structures of the bank.% of workloads that exhibit PLSL. %However, if the read queue is empty during the address selection, \tech~randomly selects a row from the list of rows that contain the overwritten content. %Furthermore, when there is only one memory location to select from, \tech~\emph{always} select that location, despite any potential memory partition-level conflicts arising due to the requests in the read queue. %In this way, the latency and energy of the write request is reduced.%By doing so, \tech~reduces   
%concurrent read and write requests \changed{originally directed} to the same memory partition to be scheduled in parallel, exploiting the partition-level parallelism in PCM. 
%\tech~implements two types of address translation, which are described next.
%In this section, we describe how address translation is achieved using the lookup table. 
%Without loss of generality, we assume the read and write requests are at the granularity of a memory line, which is the same size as a cache line. 
%We introduce two access techniques for the lookup table -- one based on indirection, and another one based on content search. 
%These are described next.
%We propose two flavors of indirection as described next. 
%The memory controller maintains a table to record all such address translations.
%As write requests are continuously re-mapped, \tech~periodically invalidates entries from the table and re-initializes \emph{unused} memory locations with all-zeros or all-ones so that future write requests can be serviced utilizing them. 

% \iscachanged{We observe that workloads exploit different partitions in PCM during execution. However, only a few partitions are accessed within small sub-intervals of the execution duration. To illustrate this, in Figure \ref{fig:part}, we plot the utilization of PCM partitions that a workload accesses during its execution. We report results for 16 workloads, which we describe in detail in Section \ref{sec:evaluation}. Additionally, we report the \emph{maximum} number of \emph{different} partitions that are accessed within sub-intervals of 64 requests (the size of our read-write queue inside the memory controller). We make the following observations. First, for workloads such as namd and mg, $\approx30$ different partitions are accessed during execution, while for workloads such as nab, only 5 partitions are accessed. Second, only a few different partitions are accessed within the sub-intervals for most workloads. For the evaluated workloads, we observe that within this sub-interval most workloads access between 2 to 4 different partitions only. We call this form of access locality in a workload as the \emph{partition-level spatial locality}. If we can cache the address translation table for only the accessed partitions within a sub-interval, and keep the full address translation table in PCM, then we can reduce \tech{}'s area overhead significantly. This is precisely the approach we adopt for \tech{}.}
% %\iscachanged{We observe that a modern PCM bank is implemented as a collection of \emph{partitions} that operate mostly \emph{independently} while \emph{sharing} a few global peripheral structures, which include the sense amplifiers (to read) and the write drivers (to write). A memory controller exploit these partitions when scheduling read and write requests within workload.}

% \begin{figure}[h!]
% 	\centering
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/part.pdf}}
% 	\caption{Utilization of PCM's partitions.}
% 	\label{fig:part}
% \end{figure}

% \iscachanged{In Figure \ref{fig:att}, we illustrate the address translation mechanism of \tech{}. Requests from DRAM cache are queued inside the memory controller. For every request to be served from the queue, the memory controller first checks to see if the address translation table for the accessed partition is cached or not. If the address translation table is cached, the PCM address of the request is first translated to the appropriate physical address, and then scheduled to PCM. We note that read requests use the cached address translation to read the translated physical location in PCM, while write requests modify an existing translation or create a new entry in the cached address translation table to overwrite all-zeros or all-ones content. To track these changes, the memory controller maintains a single bit to indicate if the cached address translation table is modified due to a request.}
% %If the address translation table for request'spartitions accessed by the requests is already cached inside the memory controller, the address is }



% \iscachanged{If however, the address translation table of a request's partition is not cached, the memory controller must fetch the address translation table for the partition from PCM and then schedule the request. This will generate extra PCM read requests to read the correct content of the address translation table. Additionally, if the cached address translation table is updated when serving one of the previous requests, then the updated address translation table needs to be saved to PCM for future translations. This will generate PCM write requests. To minimize the number of PCM transactions due to the address translation mechanism, we propose to exploit a workload's characteristics (i.e., Figure \ref{fig:part}) to cache address translations for only the partitions accessed by requests in the queue. For this purpose, we evict the address translation table for the least frequently used partition to make space for an incoming address translation table of a non-cached partition. To support our cached-address translation (CAT) policy, we propose the following two simplifications:}

% \begin{itemize}
% 	\item \iscachanged{We propose to allocate a separate PCM partition to store all address translation tables. By doing so, our memory controller can schedule reading from or writing to these tables alongside regular PCM read and write requests exploiting the partition-level parallelism in PCM banks \cite{villa2018pcm,lung2016double}}.
% 	\item \iscachanged{We disable \tech{}'s address translation for requests to read from and write to the address translation tables.}
% \end{itemize}


%We reason that 
%\tech~implements indirection-based address tra\-nslation mechanism. To facilitate this, we organize AT as fully associative structure indexed using the address of a write request (i.e., the write address). Each AT entry contains the physical address where the write address is mapped.
%The area overhead of the AT and ST combined is 72KB per each 1GB PCM bank (see Section \ref{sec:area}).
%To reduce the area overhead of AT, \tech~also implements an alternative content-based address translation mechanism (CAT) with a fixed-size AT. 
%Each AT entry stores the write address as well as the translated physical address.
%An important question to this end is how to select, which of the write requests will be redirected.
%We propose to exploit application characteristics in making such decision.
%We observe that for many workloads, over 80\% of the write requests are directed to only 20\% of the memory locations.
%This is also reported in recent works\cite{yoon2015efficient}.
%\changed{To incorporate this observation, \tech~keeps track of the write requests. Only the write-intensive physical locations in PCM are accommodated in the AT.}
%We report the area-performance tradeoffs of our CAT-based \tech~for different sizes of AT in Section \ref{sec:area}.

%\noindent\textbf{\emph{Indirection Based Translation:}}
%%We describe a fully associative flavor of indirection, where a write address can be mapped to any physical address in the PCM.
%We illustrate this in Figure \ref{fig:indirection}.
%The write request with address 0x0036 and data 0xC001 (\ding[1]{182}) is to be serviced.
%Based on the data, we see that overwriting all-zeros is energy efficient.
%%We describe address translation assuming overwriting all zeros is energy efficient for this write data.
%From the status table (ST) we see that the physical address 0x12A8 contains all-zeros (status = `10'). %This address is fet (\ding[1]{183}).
%We update the address table (AT) to store this physical address 0x12A8 at the location indexed by the write address 0x0036 (\ding[1]{184}).
%The write request is redirected to this physical address (\ding[1]{185}) and is serviced by overwriting the content with the write data (\ding[1]{186}).
%
%%request can be redirected to any memory location in the PCM that has all zeros or all ones.
%%The lookup table in this case is indexed by the write address.
%%Figure \ref{fig:indirection} shows an example indirection based address translation.
%%During a cache writeback or writethrough, a write request is generated. 
%%In this figure, the write request is to overwrite the content in address 0x0036 with data 0xAA00 (\ding[1]{182}).
%%The status register is analyzed to find a memory location that is initialized to all zeros, assuming overwriting all zeros is more energy efficient for this write data than overwriting all ones.
%%In the example, the memory location at address 0x12A8 contains all zeros (\ding[1]{183}).
%%The lookup table is next updated to store this physical address 0x12A8 at the location indexed by the write address 0x0036 (\ding[1]{184}).
%%The write request is now redirected to this physical address (\ding[1]{185}) and is serviced by overwriting the content with the write data (\ding[1]{186}).
%
%\begin{figure}[h!]
%	\centering
%	\centerline{\includegraphics[width=0.99\columnwidth]{images/indirection.pdf}}
%	\caption{Indirection based address translation.}
%	\label{fig:indirection}
%\end{figure}
%
%%The area overhead of indirection-based address translation is.
%%\begin{equation}
%%\label{eq:iat_lut_overhead}
%%\scriptsize A_{\text{LUT}} = N(\log N + 1)~~~~\text{//for AT}
%%\end{equation} 
%%\begin{equation*}
%%\label{eq:iat_status_table}
%%\scriptsize A_{\text{ST}} = 2N~~~~~~~~~~~~~~~~\text{//for ST}
%%\end{equation*} 
%%\begin{equation*}
%%\label{eq:iat_total}
%%\scriptsize A_{\text{indirection}} = A_{\text{LUT}} + A_{\text{ST}} = N(\log N + 3)
%%\end{equation*} 
%%where an AT entry needs $\log N$ bits to store the physical address and a single bit to validate the translation. 
%%The status table entry contains 1 bit to indicate whether the memory location is initialized and 1 bit to indicate if the content is all zeros or all ones.
%
%\noindent\textbf{\emph{Content Addressable Translation:}}
%In this type of addressing, a fixed size AT is used to perform the address translation. Unlike the indirection-based addressing, each AT entry stores the write address as well as the translated physical address.
%Content addressable translation allows redirecting only some of the PCM write requests in a workload. An important question to this end is how to select which of the write requests will be redirected.
%We propose to exploit application characteristics in making such decision.
%We observe that for most applications, over 80\% of the write requests are accounted for by 20\% of the memory locations in PCM.
%This is also discussed in recent works\cite{yoon2015efficient}.
%Our \tech~monitors the memory write access requests and use address translations only for the write-intensive memory locations.


%We illustrate this in Figure \ref{fig:cat}.
%%To reduce the area overhead of the lookup table, we propose an alternative content addressable address translation.
%The high level idea is to use a fixed size AT to perform address translation.
%A lookup table entry in this case contains both the write address and the physical address to which it is mapped. 
%We illustrate this in Figure \ref{fig:cat}.
%% shows the working principle of our content addressable translation.
%After identifying the data pattern to overwrite (all zeros in this example), the status table is searched to identify the physical address containing this data pattern (\ding[1]{183}).
%In this example, the physical address is 0x12A8.
%The write address is compared with all the write addresses stored in the lookup table to see if an entry exists for this write address.
%If found, the entry is updated to record the new physical address (\ding[1]{184}).
%Otherwise, a new entry is created for this mapping by replacing an entry.
%We use least recently used (LRU) replacement policy and dedicate few bits per lookup table entry to facilitate this.
%This however, increases the complexity of restoring the content of the replaced mapping to its original location.
%One way to overcome this is to exploit application characteristics.
%We observe that for most applications, over 80\% of the write requests are accounted for by 20\% of the memory locations in PCM.
%This is also discussed in recent works\cite{yoon2015efficient}.
%To exploit application characteristics for address translation, we propose to monitor the memory write access requests and use address translations only for the write-intensive memory locations.
%%In addition to the two addresses, a lookup table entry also contains few bits to facilitate replacement.
%%In this case, we use least recently used replacement policy.
%
%%To maintain data correctness after, once a write address translation entry is replaced in the lookup table to make space for a new translation, the write data in the physical address is written back to the write address.
%%In the example of Figure \ref{fig:cat}, if the highlighted entry is to be replaced by a new translation during a write request, the memory controller will issue the following two new requests before servicing the write.
%%\begin{itemize}
%%	\item rd\_data $\leftarrow$ \textbf{Read} 0x12A8
%%	\item \textbf{Write} 0x0036 rd\_data
%%\end{itemize}
%
%\begin{figure}[h!]
%	\centering
%	\centerline{\includegraphics[width=0.99\columnwidth]{images/cat.pdf}}
%	\caption{Content addressable translation.}
%	\label{fig:cat}
%\end{figure}
%
%Assuming the lookup table contains $M$ entries, the area overhead of the content addressable translation is
%\begin{equation}
%\label{eq:cat_lut_overhead}
%\scriptsize A_{\text{LUT}} = M(2\log N + L)~~~~\text{//for the lookup table}
%\end{equation} 
%\begin{equation*}
%\label{eq:cat_status_table}
%\scriptsize A_{\text{ST}} = 2N~~~~~~~~~~~~~~~~~~~~~~~\text{//for the status table}
%\end{equation*} 
%\begin{equation*}
%\label{eq:cat_total}
%\scriptsize A_{\text{total}} = A_{\text{LUT}} + A_{\text{ST}} = 2N + M(2\log N + L)
%\end{equation*} 
%where the lookup table entry contains $\log N$ bits each for the two addresses and $L$ bits to track the least recently used entry.

%Comparing Equations \ref{eq:iat_lut_overhead} with \ref{eq:cat_lut_overhead} we can observe that indirection based addressing has higher area overhead than content addressable one. However, the complexity of the latter policy is higher.
%Content addressable technique has lower overhead than indirection-based technique. However, the complexity of the latter is higher than the former.
%We evaluate the tradeoff in Section \ref{sec:results}.
%\newpage

%One way to reduce the complexity of content addressable translation is to exploit the application characteristics.
%We observe that over 80\% of the write requests are accounted for by 20\% of the memory locations in PCM.
%This is also observed in recent works \cite{yoon2015efficient}.
%To exploit this observation, we propose to monitor the memory access patterns and use address translations only for the write-intensive memory locations.

%\subsection{Scheduling Re-Initialization of Unused \\Memory Locations in \tech}

==> sections/merge_later.tex <==
\subsection{System Configuration}
To evaluate \tech{}, we designed a cycle-accurate DRAM-PCM hybrid memory simulator with the following:
\begin{itemize}
	\item A cycle-level in-house x86 multi-core simulator, whose front-end  is based on Pin~\cite{LukPin}. We configure this to simulate 8 out-of-order cores.
	\item A main memory simulator, closely matching the JEDEC Nonvolatile Dual In-line Memory Module (NVDIMM)-N/F/P Specifications~\cite{jedecnvdimm2017}. This simulator is composed of Ramulator~\cite{kim2016ramulator}, to simulate DRAM, and a cycle-level PCM simulator based on NVMain~\cite{poremba2015nvmain}. 
	%DRAMPower \cite{chandrasekar2012drampower} is used to estimate power consumption of eDRAM.
	\item Power and latency for DRAM and PCM are based on Intel/Micron's 3D Xpoint specification~\cite{bourzac2017has,villa2018pcm}. Energy is modeled for DRAM using DRAMPower~\cite{chandrasekar2012drampower} and for PCM using NVMain, with parameters from~\cite{villa2018pcm}.
\end{itemize}
%We use an in-house cycle-level PCM simulator, which interfaces with Gem5\cite{binkert2011gem5} multicore simulator.
%Similar to prior works\cite{dhiman2009pdram}, we assume hybrid DRAM-PCM architecture with an on-chip eDRAM L3 cache similar to that of the IBM POWER7 processor\cite{kalla2010power7}. 
%A 16GB PCM is used as the main memory with latency and energy parameters based on 90nm PCM design \cite{LeeISCA2009}.
%Note that the peripheral circuitry latency and energy are accounted for when accessing the row buffer, which occurs on every access.
Table \ref{tab:config} shows our simulation parameters. The memory controller implements a 16-entry read queue, a 16-entry write queue, and an 8-entry InitQ per each bank.

 %Additionally, a separate 8-entry initialization queue is implemented for \tech. 
%The status and address tables are also implemented inside the memory controller.

\subsection{Evaluated Workloads}
We evaluate the following workloads.
\begin{itemize}
	\item %\emph{Table \ref{tab:spec}:} 
	8 SPEC CPU2017 workloads~\cite{bucek2018spec}: bwaves, cactusBSSN, leela, mcf, omnetpp, parset, roms, and xalancbmk.
	2 NAS Parallel workloads~\cite{bailey1991parallel}: bt and ua.
	10 TensorFlow machine learning workloads~\cite{tfex}: mlp, cnn, gan, rnn, dcgan, bidirectional rnn (bi\_rnn), autoencoder (autoenc), logistic regression (lr), random forest (rf), and word2vec.
\end{itemize}

All workloads are executed for 10 billion instructions. Figure~\ref{fig:mpki} plots the eDRAM Misses Per Kilo Instruction (MPKI) of the evaluated workloads.
For other workloads with low MPKI (not reported in Section~\ref{sec:results}), \tech{} neither significantly improves nor hurts performance and energy.

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/mpki.pdf}}
	\vspace{-10pt}
	\caption{eDRAM cache MPKI for the evaluated workloads.}
	\vspace{-10pt}
	\label{fig:mpki}
\end{figure}

\subsection{Evaluated Systems}
We evaluate the following systems.%previously-proposed state-of-the-art systems for PCM.
\begin{itemize}
	\item \emph{Baseline}~\cite{LeeISCA2009}, which services PCM writes by overwriting \emph{unknown} content.
	\item \emph{PreSET}~\cite{QureshiISCA12}, which services PCM writes by \emph{always} overwriting all-1s. %For this purpose, the preset operation of a memory location is initiated as soon as a write to the eDRAM cache line is performed.
	\item \emph{Flip-N-Write}~\cite{cho2009flip}, which services PCM writes by \emph{finding out} the memory content using additional reads and programming only bits that are different from the write data. %using read before write methodology, where a memory location is first read before overwriting its content.
	\item \emph{\tech}, which redirects write requests to overwrite all-0s or all-1s content, depending on the write data. 
\end{itemize}
%We evaluate two flavors of our \tech~mechanism.
%\begin{itemize}
%	\item \emph{\tech:} This is our baseline system for redirecting write requests to overwrite all-zeros and all-ones content. %with fully associative address translation. Scheduling of reinitialization operations are performed only when RdQ and WrQ are both empty.
%	\item \emph{\tech-CAT:} This is our baseline technique with content addressable translation.
	%\item \emph{\tech-PLP:} This is the \tech~system which exploits partition-level parallelism (PLP) in PCM banks.
%\end{itemize}

\begin{table}[h!]
	\centering
	\vspace{-5pt}
	\caption{Major Simulation Parameters.}
	\label{tab:config}
	\vspace{-5pt}
	{\fontsize{8}{10}\selectfont
		\begin{tabular}{lp{5cm}}
			\hline
			Processor & 8 cores per socket, 3.32 GHz, out-of-order\\
			\hline
			L1 cache & Private 32KB per core, 8-way\\
			\hline
			L2 cache & Private 512KB per core, 8-way\\
			\hline
			L3 cache & Shared 8MB, 16-way\\
			\hline
			eDRAM cache & Shared 64MB per socket, 16-way, on-chip\\
			\hline
			\multirow{5}{*}{Main memory} & 128GB PCM. \\
			& 4 channels, 4 ranks/channel, 8 banks/rank, 8 partitions/bank, 128 tiles/partition, 4096 rows/tile.\\
			& Memory interface = DDR4\\
			& Memory clock = 1066MHz\\
			& PCM Timings = See Table \ref{tab:min_max_latency}\\
			\hline
% 			\multirow{4}{*}{Memory Timing} & PCM cell read: 11 cycles\\
% 			& PCM cell SET: 24 cycles\\
% 			& PCM cell RESET: 18 cycles\\
% 			& Program \& Verify: 35 cycles\\
% 			\hline
% 			\multirow{3}{*}{Memory Energy} & read: 2.0pJ/bit\\
% 			& SET: 13.5pJ/bit\\
% 			& RESET: 19.2pJ/bit\\
% 			\hline
	\end{tabular}}
\end{table}

\vspace{-5pt}

% \iscachanged{We chose these benchmarks because they have at least 1 memory access per 1000 instructions out of the 64MB on-chip eDRAM cache. In Figure \ref{fig:rw_distribute}, we report the read and write distribution of the PCM requests generated from these workloads. We make the following observation. Some workloads such as mcf, namd, povray, omnetpp, xalancbml, imagick, leela, and nab have very little or no write requests. For these workloads, the performance of all our evaluated systems are the same. For other workloads, where there are significant percentage of write requests, we see performance improvement using our \tech{} system (Section \ref{sec:results}).}


% \begin{figure}[h!]
% 	\centering
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/rw_distribute.pdf}}
% 	\caption{Distribution of PCM read and write requests for each of our workloads.}
% 	\label{fig:rw_distribute}
% \end{figure}

%We perform timing simulations for 2 million memory accesses for the baseline system.
%Columns 3 and 4 in Tables \ref{tab:spec}, \ref{tab:nas}, and \ref{tab:ml} report respectively, the percentage of memory cycles a PCM bank is servicing read and write accesses. Column 5 reports the read-to-write ratio for these workloads.
%\begin{table}[h!]
%	\centering
%	{\fontsize{6}{12}\selectfont
%		\begin{tabular}{|c|l||c|c|c|}
%			\hline
%			\multirow{2}{*}{\textbf{Workload}} & \multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{2}{|c|}{\textbf{Bank Utilization}} & \textbf{Read-to}\\
%			\cline{3-4}
%			& & \textbf{Reads} & \textbf{Writes} & \textbf{Write}\\
%			\hline
%			\hline
%			milc & 16 copies of milc & 30\% & 10\% & 3:1\\
%			zeusmp & 16 copies of zeusmp & 16\% & 42\% & 1:2.6\\
%			leslie3d & 16 copies of leslie3d & 15\% & 26\% & 1:1.7\\
%			sjeng & 16 copies of sjeng & 60\% & 15\% & 4:1\\
%			GemsFDTD & 16 copies of GemsFDTD & 60\% & 36\% & 1.7:1\\
%			libquantum & 16 copies of libquantum & 15\% & 0.002\% & 750:1\\
%			lbm & 16 copies of lbm & 33\% & 40\% & 1:1.2\\
%			omnetpp & 16 copies of omnetpp & 92\% & 3\% & 30.7:1\\
%			astar & 16 copies of astar & 10\% & 20\% & 1:2\\
%			xalancbmk & 16 copies of xalancbmk & 82\% & 13\% & 6.3:1\\
%			\hline
%	\end{tabular}}
%	\caption{PCM bank utilization for ten workloads from the SPEC CPU2006 suite.}
%	\label{tab:spec}
%\end{table}
%
%\begin{table}[h!]
%	\centering
%	\setlength{\tabcolsep}{4pt}
%	{\fontsize{6}{12}\selectfont
%		\begin{tabular}{|c|l||c|c|c|}
%			\hline
%			\multirow{2}{*}{\textbf{Workload}} & \multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{2}{|c|}{\textbf{Bank Utilization}} & \textbf{Read-to}\\
%			\cline{3-4}
%			& & \textbf{Reads} & \textbf{Writes} & \textbf{Write}\\
%			\hline
%			\hline
%			conjgrad & 8 copies of conjugate gradient & 36\% & 60\% & 1:1.7\\
%			intsort & 8 copies of integer sort & 27\% & 69\% & 1:2.5\\
%			\hline
%	\end{tabular}}
%	\caption{PCM bank utilization for two workloads from the NAS Parallel Benchmark suite.}
%	\label{tab:nas}
%\end{table}
%
%\begin{table}[h!]
%	\centering
%	\setlength{\tabcolsep}{2pt}
%	{\fontsize{6}{12}\selectfont
%		\begin{tabular}{|c|l||c|c|c|}
%			\hline
%			\multirow{2}{*}{\textbf{Workload}} & \multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{2}{|c|}{\textbf{Bank Utilization}} & \textbf{Read-to}\\
%			\cline{3-4}
%			& & \textbf{Reads} & \textbf{Writes} & \textbf{Write}\\
%			\hline
%			\hline
%			km & 1 copy of K-means clustering & 72\% & 23\% & 3.1:1\\
%			mlp & 1 copy of multi-layer perceptron & 87\% & 8\% & 10.9:1\\
%			ql & 1 copy of Q learning & 86\% & 9\% & 9.5:1\\
%			rf & 1 copy of random forest classifier & 51\% & 45\% & 1.1:1\\
%			svm & 1 copy of support vector machine & 61\% & 34\% & 1.8:1\\
%			\hline
%	\end{tabular}}
%	\caption{PCM bank utilization for 5 machine learning applications.}
%	\label{tab:ml}
%\end{table}

%We make the following observations from the bank utilization data in Table \ref{tab:spec} for the SPEC workloads.

%First, some workloads like astar and leslie3d have high idle periods (41.7\% and 32.7\%, respectively) despite having modest write accesses to the PCM.
%For these workloads a PCM location cached in the eDRAM cache is modified multiple times before eviction.
%We observe that the number of processor cycles between the first time a memory location in the eDRAM cache is modified and its actual eviction from the cache is in the order of few millions, providing opportunity for the PreSET technique to program the cached location to all ones before overwriting it during writeback.
%The latency of a preset operation is overlapped with other write accesses causing very little impact on the system performance for these workloads.

%Second, other workloads like sjeng and lbm have low idle periods (3.0\% and 2.6\%).
%This is also the case for the two workloads from the NAS benchmark suite and the machine learning suite.
%For these workloads, the latency of preset operations interfere with the read and write accesses of PCM causing significant performance degradation as we show in Section \ref{sec:perf}.

%\begin{figure*}[h!]
%	\centering
%	\centerline{\includegraphics[width=1.99\columnwidth]{images/total_energy.pdf}}
%	\caption{Total energy reduction over baseline for 17 workloads (listed in Tables \ref{tab:spec}-\ref{tab:ml}).}
%	\label{fig:energy}
%\end{figure*}


\subsection{Figures of Merit}
We report the following figures of merit in this work.

%\vspace{-5pt}

\begin{itemize}
	\item \emph{Access Latency:} The sum of queuing delay and service latency, averaged across all PCM accesses. 
	\item \emph{System Energy Consumption:} The sum of DRAM and PCM energy for all accesses.% for a workload
	\item \emph{Execution Time:} The time to complete a workload.
	%\item \emph{text}
\end{itemize}
\vspace{0.3pt}

%\vspace{-10pt}

\begin{figure*}[b!]
	\centering
	\vspace{-10pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/execution_time.pdf}}
	\vspace{-10pt}
	\caption{Execution time normalized to Baseline for the evaluated workloads.}
	\vspace{-10pt}
	\label{fig:extime}
\end{figure*}

\begin{figure*}[b!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/write_distribution.pdf}}
	\vspace{-10pt}
	\caption{Total PCM writes distributed into overwriting all-0s, all-1s, and unknown content in \tech{}, compared to overwriting all-1s and unknown content in PreSET \cite{QureshiISCA12}.}
	\vspace{-10pt}
	\label{fig:write_distribution}
\end{figure*}

\begin{figure*}[b!]
	\centering
	\vspace{-10pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/access_latency.pdf}}
	\vspace{-10pt}
	\caption{Access latency normalized to Baseline for the evaluated workloads.}
	\vspace{-10pt}
	\label{fig:actime}
\end{figure*}

\begin{figure*}[b!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/energy_consumption.pdf}}
	\vspace{-10pt}
	\caption{Energy consumption normalized to Baseline for the evaluated workloads.}
	\vspace{-10pt}
	\label{fig:energy}
\end{figure*}


==> sections/tradeoff.tex <==
\mc{To evaluate the performance and energy trade-off performed by \tech{} in response to the write data, we designed a microbenchmark, where the same write data is used for every PCM write access. We ran the microbenchmark repeatedly while increasing the fraction of set bits in the write data every time.
Figure \ref{fig:tradeoff} plots the execution time and energy of \tech{} normalized to Baseline when increasing the fraction of set bits from 0\% (write data is all-0s) to 100\% (write data is all-1s).}
%, where the fraction of SET bits in write data is increased from 0\% (write data is all-0s) to 100\% (write data is all-1s).
We make the following two main observations.

\begin{figure}[h!]
	\centering
	\centerline{\includegraphics[width=1.01\columnwidth]{images/tradeoff.pdf}}
	\vspace{-10pt}
	\caption{\mc{Execution time and energy of \tech{} normalized to Baseline with increasing fraction of SET bits in the write data of a microbenchmark.}}
	\label{fig:tradeoff}
\end{figure}

\mc{
First, as the fraction of set bits in write data is increased, the energy consumption increases, reaching a peak at around 60\%, and then decreases. This is due to the energy difference of SET and RESET operations, which we have analyzed in Section~\ref{sec:quantifying_perf} and illustrated in our Observation 1 in Figure~\ref{fig:set_reset_energy}. \tech{} lowers the energy consumption by switching from only SET operations (overwriting all-0s) to only RESET operations (overwriting all-1s) as the fraction of SET bits in the write data exceeds 60\%.
Second, as SET operation in PCM has lower latency than RESET operation (see Table~\ref{tab:min_max_latency}), switching to only RESET operations also leads to lower execution time, i.e., higher performance.
}
